Survey of Methods for Solving Systems of Nonlinear Equations, Part II: Optimization Based Approaches

This paper presents a comprehensive survey of methods which can be utilized to search for solutions to systems of nonlinear equations (SNEs). Our objectives with this survey are to synthesize pertinent literature in this field by presenting a thorough description and analysis of the known methods capable of finding one or many solutions to SNEs, and to assist interested readers seeking to identify solution techniques which are well suited for solving the various classes of SNEs which one may encounter in real world applications. To accomplish these objectives, we present a multi-part survey. In part one, we focused on root-finding approaches which can be used to search for solutions to a SNE without transforming it into an optimization problem. In part two, we introduce the various transformations which have been utilized to transform a SNE into an optimization problem, and we discuss optimization algorithms which can then be used to search for solutions. We emphasize the important characteristics of each method, and we discuss promising directions for future research. In part three, we will present a robust quantitative comparative analysis of methods capable of searching for solutions to SNEs.

==> symbolic_computation.tex <==
% \section{Symbolic Computation}

Exact algorithmic methods for solving systems of nonlinear polynomial equations have been developed in the realm of \textit{Symbolic Computation}, also called \textit{Computational Algebra}, or \textit{Computer Algebra}. Broadly speaking, this particular subarea of Symbolic Computation can in fact be interpreted as a constructive version of some parts of the well-established mathematical 
theories of \textit{Commutative Algebra} and \textit{Algebraic Geometry}. We begin this section by a brief presentation (via examples) of the main Symbolic Computation methods for solving systems of nonlinear polynomial equations, namely \textit{resultants} and \textit{Gr{\"o}bner bases}.
We end this section by citing a number of books that discuss extensively all the developments in the area of Symbolic Computation exact methods for solving systems of nonlinear polynomial equations. 

\subsubsection{Resultants}\phantom{}\vspace*{0.1cm}

\noindent
Historically, the theory of resultants was developed with the aim to provide a systematic means of elimination of variables/unknowns from a system of nonlinear polynomial equations. 

The resultant of two univariate polynomials of degrees $m$, $n$ respectively, 
\[
p(x)=p_m x^m + \cdots + p_1 + p_0, \kern0.8cm q(x)=q_n x^n + \cdots + q_1 + q_0,
\]
is defined as the determinant of the $(n+m)\times(n+m)$ Sylvester matrix associated to $p(x)$ and $q(x)$, namely:
\[
    {\rm res}_x\bigl(p(x),q(x)\bigr) = 
    {\rm det} \left[
    \begin{array}{llll}
         a_m &  a_{m-1} &          & \\
          0  & a_m     & a_{m-1}  & \\
          0  &  0      & a_m      & a_{m-1} \\
          0  &  0      & 0        & a_m     \\
         b_n & b_{n-1} &          & \\
          0  & b_n     & b_{n-1}  & \\
          0  &  0      & b_n      & b_{n-1} \\
          0  &  0      & 0        & b_n \\ 
    \end{array}
    \right] .
\]
One of the main properties of the resultant is that it is equal to zero, if and only if the two polynomials have a common root.

The resultant of two bivariate polynomials $p=p(x,y)$,\kern0.1cm $q=q(x,y)$ with respect to the variable $x$, or with respect to the variable $y$, is the determinant of their associated Sylvester matrix, when $p$ and $q$ are considered as polynomials in $x$, or in $y$ respectively. 

Let us illustrate the concept of the resultant by a simple but instructive example. 
\begin{example}{\em
Consider the system of two polynomials $f_1(x_1,x_2) = 0, f_2(x_1,x_1) = 0$ in two variables $x_1,x_2$, given by:
\begin{equation}
    \begin{array}{l}
         f_1(x_1,x_2) = x_1^2+x_2^2-1, \\[0.1cm]
         f_2(x_1,x_2) = x_1-x_2-1. \\ 
    \end{array}
    \label{SymbolicComputation:Resultants:example}
\end{equation}
The resultant of $f_1,f_2$, with respect to $x_1$  is the determinant of their $3\times 3$ Sylvester matrix when considered as polynomials in $x_1$, namely, $f_1 = 1 \cdot x_1^2 + 0 \cdot x_1 + (x_2^2-1)$, $f_2 = 1 \cdot x_1 +(-x_2 - 1)$, 
$$
{\rm res}_{x_1}(f_1,f_2) = \det 
 \left[ \begin {array}{ccc} 1&0&{{\it x_2}}^{2}-1\\ \noalign{\medskip}1&-
{\it x_2}-1&0\\ \noalign{\medskip}0&1&-{\it x_2}-1\end {array} \right]
= 2x_2^2 + 2x_2 .
$$
By factorizing the resultant and setting it equal to zero, we obtain $x_2=0$ and $x_2= -1$. By substituting each of these two values of $x_2$ back into (\ref{SymbolicComputation:Resultants:example}), we obtain the corresponding values of $x_1$ as: $x_1=1$ and $x_1=0$. Therefore, we conclude that the system (\ref{SymbolicComputation:Resultants:example}) possesses the two solutions:
\[
    (x_1=1,\,\,x_2=0),\kern0.2cm (x_1=0,\,\,x_2=-1) , 
\]
which can easily be verified to be correct. In terms of geometric interpretation, the first equation $f_1(x_1,x_2)$ represent the unit circle and the second equation $f_1(x_1,x_2)$ represents a straight line, that intersects the unit circle. The two solutions of the system (\ref{SymbolicComputation:Resultants:example}) are the two points of intersection of the (red) unit circle and this (green) straight line in Figure 2 below. 
\begin{figure}[h]\label{fig4} 
\centering
 %\includegraphics[width=\linewidth]{NSE_example_resultants.png}
 \includegraphics[width=7.5cm]{NSE_example_resultants.png}
  \caption{Geometric interpretation of System (\ref{SymbolicComputation:Resultants:example}) }
\end{figure}
}\end{example}

\subsubsection{Gr{\"o}bner bases}\phantom{}\vspace*{0.1cm}

\noindent
The theory of Gr{\"o}bner bases was developed as a multivariate analogue of the classical \textit{Gaussian elimination} for systems of linear equations. Again we illustrate the concept with an example and refer to the aforementioned books for additional details and technicalities. 
\begin{example}{\em
Consider the system of three polynomials $f_1(x_1,x_2,x_3) = 0$,\, $f_2(x_1,x_2,x_3) = 0$,\, $f_3(x_1,x_2,x_3) = 0$\, in three variables $x_1,x_2,x_3$, given by:
\begin{equation}
    \begin{array}{l}
         f_1(x_1,x_2,x_3) = x_1^{2}+x_2 x_3 -2, \\ [0.1cm]
         f_2(x_1,x_2,x_3) = x_1 x_3 +x_2^{2}-3, \\ [0.1cm]
         f_3(x_1,x_2,x_3) = x_1 x_2 +x_3^{2}-5. \\
    \end{array}
    \label{SymbolicComputation:Groebner:example}
\end{equation}
The lexicographical Gr{\"o}bner basis of the ideal generated by these three polynomials, with respect to the lexicographical ordering induced by $x_2 > x_1 > x_3$ is given by the three polynomials: 
\begin{equation}
    \begin{array}{l}
    8 x_2^{8}-60 x_2^{6}+142 x_2^{4}-172 x_2^{2}+1, \\[0.1cm]
88 x_2^{7}-680 x_2^{5}+1674 x_2^{3}-2081 x_2 +117 x_1, \\[0.1cm]
152 x_2^{7}-1132 x_2^{5}+2700 x_2^{3}-3403 x_2 +117 x_3. \\
    \end{array}
    \label{GB_plex}
\end{equation}
Now we notice that the first polynomial in (\ref{GB_plex}) depends only on $x_2$ and is of degree $8$. In addition, the second polynomial in (\ref{GB_plex}) depends linearly on $x_1$ and the third polynomial in (\ref{GB_plex}) depends linearly on $x_3$. This allows us to express $x_1$ and $x_3$ as polynomials in $x_2$. Therefore, the solution process starts by finding the 8 roots of the first polynomial in (\ref{GB_plex}) and for each one of those roots, we find the unique values of $x_1$ and $x_3$, given by the last two polynomials in (\ref{GB_plex}). Here are the eight complex roots (four real roots and two pairs of complex conjugate roots) of the first polynomial in (\ref{GB_plex})
$$
\begin{array}{l}
-2.16624183202470499 \\[0.1cm]
\kern0.22cm 2.16624183202470499 \\[0.1cm]
-0.07643337499454630 \\[0.1cm] 
\kern0.22cm 0.07643337499454630  \\[0.1cm]
-1.329681781358029 - 0.606033421098925 \,\mathrm{i} \\[0.1cm]
-1.329681781358029 + 0.606033421098925 \,\mathrm{i} \\[0.1cm]
\kern0.22cm 1.329681781358029 -0.606033421098925 \,\mathrm{i} \\[0.1cm]
\kern0.22cm 1.329681781358029 + 0.606033421098925 \,\mathrm{i} \\
\end{array}
$$
Note that the four real roots and the four complex roots come in pairs of the form $(r,-r)$, a consequence of the fact that the first polynomial in (\ref{GB_plex}) contains only even powers of $x_2$. The presence of only even powers of the indeterminate $x_2$ in the first polynomial in (\ref{GB_plex}) is captured by the fact that the order of the Galois group of this polynomial is smaller than the order of the Galois group of a more ``random/generic'' polynomial of degree $8$. 
}\end{example}
A very readable, self-contained and pedagogical introduction to  Gr{\"o}bner bases can be found in chapter 10 of \cite{GeddesCzaporLabahn:1992}.

\subsubsection{Symbolic computation software systems}\phantom{}\vspace*{0.1cm}
%software systems review

One of the major outcomes of the research area of Symbolic Computation (Computer Algebra) in the past few decades, 
is the advent of the so-called Computer Algebra Systems (CAS).
A CAS is defined as a piece of mathematical software that makes advanced functionalities available to the user, in a transparent manner. Such advanced functionalities include univariate and multivariate polynomial factorization, primality testing, integer factorization, root finding, numerical and exact integration, visualization, number theory, linear algebra, commutative algebra, commutative and non-commutative settings, tools for optimization, graph theory, group theory, coding theory, combinatorics, discrete mathematics and so forth.     
There is a number of commercial and free (open source) CAS available today. Some of the most well-known early CAS (such as Axiom and Macsyma) are largely deprecated today. We focus our attention on those CAS that currently feature a significant user base. We note that CAS are used by millions of research mathematicians, physicists, chemists, astronomers, engineers, practitioners and educators at academic, public, private and government institutions worldwide. In what follows, we provide a brief summary of the main commercial CAS in use today.

\begin{itemize}
    \item[(a)] Maple is the flagship Canadian product in the area of mathematical software. It is produced, maintained and distributed by the company Maplesoft, based in Waterloo, Ontario, Canada \url{https://www.maplesoft.com/}. Maple features an easy-to-learn underlying programming language as well as more than $150$ additional packages that significantly expand its core functionalities.   
    \item[(b)] Magma is the flagship Australian product in the area of mathematical software. It is produced, maintained and distributed by the University of Sydney \url{http://magma.maths.usyd.edu.au/}. It provides a mathematically rigorous environment for defining and working with structures such as groups, rings, fields, modules, algebras, schemes, curves, graphs, designs, codes and many others. Magma also supports a number of databases designed to aid computational research in those areas of mathematics which are algebraic in nature.
    \item[(c)] Mathematica is a flagship American product in the area of mathematical software. It is produced, maintained and distributed by the company Wolfram Research, based in Champaign, Illinois, United States \url{https://www.wolfram.com/}. Mathematica's stated purposes include injecting computational intelligence at every level, on every project by unifying algorithms, data, notebooks, linguistics and deployment—enabling powerful workflows across desktop, cloud, server and mobile.
    \item[(d)] Matlab is a flagship American product in the area of mathematical software.  \url{https://www.mathworks.com}. It is produced, maintained and distributed by the company MathWorks, based in California, United States. MATLAB's strong points include matrix manipulations, plotting of functions and data, implementation of algorithms, creation of user interfaces, and interfacing with programs written in other languages.
\end{itemize}

Some of the most popular non-commercial mathematical software packages include Sage, Singular/Plural, CoCoA, Macaulay 2 and so forth. Each one has their own strengths and areas of particular focuses. For more information on CAS in general, we refer the interested reader to the comprehensive book \cite{Wester:1999}.

\subsubsection{Symbolic computation books}\phantom{}\vspace*{0.1cm}
%literature review

\noindent
In this section, we present a selection of books in Symbolic computation and related areas. While there is inevitably some overlap among these books, there are also different aspects of polynomial system solving and its applications discussed in each one of them.  

\begin{enumerate}
\setlength{\itemsep}{4pt}
    \item
The classic books \cite{GeddesCzaporLabahn:1992,Davenport:Siret:Tournier:1993,vzGathen:Gerhard:2013} are general references for Computer Algebra.

    \item
The series of books by Teo Mora
%\cite{Teo_Mora:EMA_I_2003},
%\cite{Teo_Mora:EMA_II_2005},
%\cite{Teo_Mora:EMA_III_2015},
%\cite{Teo_Mora:EMA_IV_2016}
\cite{Teo_Mora:EMA_I_2003, Teo_Mora:EMA_II_2005, Teo_Mora:EMA_III_2015, Teo_Mora:EMA_IV_2016}
is an encyclopedic reference to the subject of polynomial system solving.

    \item
The theory of Gr{\"o}bner bases, see 
%\cite{William_W_Adams_Philippe_Loustaunau:1994},
%\cite{Thomas_Becker_Volker_Weispfenning:1993},
%\cite{Ralf_Froberg:1997},
%\cite{Franz_Winkler:1996},
\cite{William_W_Adams_Philippe_Loustaunau:1994,%
Thomas_Becker_Volker_Weispfenning:1993,%
Ralf_Froberg:1997,%
Franz_Winkler:1996},
was initially developed by Bruno Buchberger 
and further extended by several other researchers.
The \textit{Buchberger algorithm} to compute Gr{\"o}bner bases 
of polynomial systems is implemented in every major 
Symbolic Computation software today. This includes commercial software, 
such as Maple, Magma and Mathematica and open source software, such as 
Singular \cite{Wolfram_Decker_Christoph_Lossen:2006}, 
Plural \cite{Wolfram_Decker_Gerhard_Pfister:2013}, 
CoCoA 
%\cite{Martin_Kreuzer_Lorenzo_Robbiano:2000}, 
%\cite{Martin_Kreuzer_Lorenzo_Robbiano:2005},
%\cite{Martin_Kreuzer_Lorenzo_Robbiano:2008},
%\cite{Martin_Kreuzer_Lorenzo_Robbiano:2016}
\cite{Martin_Kreuzer_Lorenzo_Robbiano:2000,% 
Martin_Kreuzer_Lorenzo_Robbiano:2005,%
Martin_Kreuzer_Lorenzo_Robbiano:2008,%
Martin_Kreuzer_Lorenzo_Robbiano:2016}
and the Macaulay2 software system \cite{Macaulay2:Grayson:Stillman}.

    \item
The book \cite{Bernd_Sturmfels:2002} discusses aspects of systems of polynomial equations from the viewpoints of computational commutative algebra, discrete geometry, elimination theory, real geometry, as well as their applications in various domains such as partial differential equations, economics, probability, and statistics. 

    \item
The book \cite{Invariant_Theory_Sturmfels:1993} and its second edition \cite{Invariant_Theory_Sturmfels:2008}, describe useful algorithmic aspects of systems with symmetries, treated using \textit{Invariant Theory}.  
The book \cite{Karin_Gatermann:2000} is concerned with 
polynomial systems with symmetries, that arise in the 
context of dynamical systems. The french-language book \cite{Elkadi:Mourrain:2007} is devoted exclusively to polynomial system solving 
methods. The french-language book \cite{AECF:2017} contains a series of chapters on polynomial system solving.

    \item
The books \cite{Algebraic_Statistics_Pistone_Riccomagno_Wynn:2001} and \cite{Algebraic_Statistics_Sullivant:2018} describe the emerging area of 
\textit{Algebraic Statistics}, 
%
while
the book \cite{Hans_J_Stetter:2004} focuses on numerical aspects of
polynomial system solving.
%
On the other hand,
the book \cite{Alicia_Dickenstein_Ioannis_Z_Emiris:2005} focuses on 
theoretical aspects of polynomial system solving.
Furthermore,
the books trilogy 
%\cite{Cox:2020:CBMS:134}, \cite{CLO_UTM_2nd_ed:2005}, \cite{CLO_UTM_4th_ed:2015} 
\cite{Cox:2020:CBMS:134,CLO_UTM_2nd_ed:2005,CLO_UTM_4th_ed:2015} 
examine the foundation of polynomial system solving from the algebraic geometry standpoint as well as the applications standpoint.
The Galois group of a polynomial is inextricably linked with the more general \textit{Galois Theory}, 
we mention the three books \cite{GALOIS:Cox:2012,GALOIS:Stewart:2015,GALOIS:Tignol:2016}. 
\end{enumerate}






